A Nonparametric Frequency Domain EM Algorithm for Time Series Classification with Applications to Spike Sorting and Macro-Economics

I propose a frequency domain adaptation of the Expectation Maximization (EM) algorithm to group a family of time series in classes of similar dynamic structure. It does this by viewing the magnitude of the discrete Fourier transform (DFT) of each signal (or power spectrum) as a probability density/mass function (pdf/pmf) on the unit circle: signals with similar dynamics have similar pdfs; distinct patterns have distinct pdfs. An advantage of this approach is that it does not rely on any parametric form of the dynamic structure, but can be used for non-parametric, robust and model-free classification. This new method works for non-stationary signals of similar shape as well as stationary signals with similar auto-correlation structure. Applications to neural spike sorting (non-stationary) and pattern-recognition in socio-economic time series (stationary) demonstrate the usefulness and wide applicability of the proposed method.

==> input/clustering.tex <==
\section{Clustering spikes}


==> input/clustering_frequency.tex <==

\section{Clustering in the complex plane}
Doing the FFT of the signal the different wave forms must be visible as ``cones'' on the complex plane, pointing in some particular direction (the important frequency); due to the way the data is collected these cones are very likely pointing towards low frequencies (something like angles greater than $\pi / 16$). 

The noise in the measurements will be apparent by a circular bivariate distributed point cloud around $(0,0)$: this is the white noise sequence.

Picking out these cones will give the clusters. 

\begin{remark}
The logarithm of the Fourier coefficients converts the ``cones'' to nice horizontal lines; much easire to cluster. Look into the complex logarithm.
\end{remark}

\begin{figure}[!t]
\centering
\makebox{\includegraphics[width=\textwidth]{images/simulated_spike_trains.png}}
\caption{\label{fig:simulated_spike_trains} (top left) the $5$ true signals $S_i(t)$ of $5$ neurons; (top right) $N$ measured signals plus noise $s_{i,t}$, $t = 1, \ldots, 46$; (bottom left) Fourier coefficients in the complex plan of all $N$ signals; (bottom right) logarithm of the Fourier coefficients.}
\end{figure}



\begin{figure}[!t]
\centering
\makebox{\includegraphics[width=\textwidth]{images/true_and_noisy.png}}
\caption{\label{fig:simulated_spike_trains} (top left) the $5$ true signals $S_i(t)$ of $5$ neurons; (top right) $N$ measured signals plus noise $s_{i,t}$, $t = 1, \ldots, 46$; (bottom left) Fourier coefficients in the complex plan of all $N$ signals; (bottom right) logarithm of the Fourier coefficients.}
\end{figure}

\begin{figure}[!t]
\centering
\makebox{\includegraphics[width=\textwidth]{images/joint_density_plot_sim.png}}
\caption{\label{fig:simulated_spike_trains} Joint density of a mixture of $10$ Gamma - von Mises distributions}
\end{figure}




\subsection{Prior knowledge/ distributions}

The higher the variance of the noise, the wider the cones on the plane ($\rightarrow$ linear models theory: $\V \beta = \sigma^2 (X'X)^{-1}$. For Fourier basis, this $X'X = I$ (orthonormal), so the width of the cone should grow linearly with the variance of the noise.)

For an iid sequence all frequencies are equally important (uniform distribition) and the disribution of the radii of the coefficients is exponential (see Brockwell and Davis).

For the signals a von Mises distribution on the frequency and a Gamma distribution for the coefficients for a given frequency would make sense, i.e.\ Fourier coefficients $a_{j} = r \exp(i \varphi)$ are random variables with the frequency $\varphi$ having a von Mises distribution\footnote{\url{https://secure.wikimedia.org/wikipedia/en/wiki/Von_Mises_distribution}}
\begin{equation}
\varphi \sim f(\lambda | \mu, \kappa) = \frac{e^{\kappa\cos(x-\mu)}}{2\pi I_0(\kappa)}
\end{equation}


Then for a given frequency, the radius of the Fourier coefficients should follow a distribution that has the exponential distribution as a special case, since for an iid sequence the distribution is exponential (Brockwell and Davis). For example the Gamma distribution would be useful (also because it's from a conjugate family)
\begin{equation}
r | \varphi \sim \Gamma(k, \theta)
\end{equation}

For a simple model just assume that radius and phase are independent. However, for this data they presumably are not: since we measure the signals only over a certain time frame (that tries to exactly match one complete waveform), very high frequencies will not be important for these series. Thus if $\varphi$ is very small, then also the radius is presumably small. Or in terms of distributions, for low frequencies I expect a more exponential distribution than for low frequencies (that's where Fourier coefficients will show up).


==> input/fourier.tex <==
\section{Fourier Analysis}
As every bounded, continuous function can be approximated arbitrarily well by Fourier polynomials of sufficiently high order (in the mean square sense), we can write each spike wave as 
\begin{equation}
S(t) = \sum_{\ell=-\infty}^{\infty} \alpha_{\ell} e^{i \ell t}, \text{ with } \alpha_{\ell} = \overline{\alpha}_{\ell},
\end{equation}
where $\overline{z} = a - ib$ is the complex conjugate of the complex number $z = a+ib$. This must hold as $S_i(t)$ is a real-valued function; thus the coefficients of the Fourier series must be complex conjugates.

The Fourier coefficients can be computed by
\begin{equation}
\alpha_{\ell} = \frac{1}{2\pi}\int_{-\pi}^{\pi} S(t) e^{-i \ell t}\, dt. 
\end{equation}
Since $S_i(t)$ and $\lbrace a_{\ell}^{(i)} \rbrace$ are also in a one-to-one relation we have
\begin{equation}
\text{ Neuron } n_i \leftrightarrow S_i(t) \leftrightarrow \boldsymbol{\alpha}^{(i)}
\end{equation}

Thus if we want to classify the signals we measure to which $n_i$ they are coming from, we can either classify the wave forms $S_i(t)$ or classify Fourier coefficients. The advantage of Fourier coefficients is that in general there will be only very few important coefficients (since the wave forms are already ``nice'' harmonics, and not random signals).

In general the function is not on $[-\pi, \pi]$: for a periodic function $f(t)$ on $[a, a+ \tau]$ the formulas become
\begin{equation}
f(x)=\sum_{\ell =-\infty}^\infty \alpha_{\ell} \cdot e^{i 2\pi \frac{\ell}{\tau} x}. 
\end{equation}
and the coefficients are
\begin{equation}
 \alpha_{\ell} = \frac{1}{\tau}\int_a^{a+\tau} f(x)\cdot e^{-i 2\pi \frac{\ell}{\tau} x}\, dx. 
\end{equation}

For measured data and for ``nice'' wave forms, the infinite sum for spike-signal $S(t)$ can be split into the important frequencies\footnote{Note that the important frequencies are not necessarily the first frequencies in $j$.} $\mathcal{K}_i$ and the noise
\begin{eqnarray}
S_i(t) &=& \sum_{\ell \in \mathcal{K}_i} \alpha_{\ell} \cdot e^{i 2\pi \frac{\ell}{\tau} t} +  \sum_{j \notin \mathcal{K}_i} a_n \cdot e^{i 2\pi \frac{\ell}{\tau} t} \\
 &=& \sum_{\ell \in \mathcal{K}_i} \alpha_{\ell} \cdot e^{i 2\pi \frac{\ell}{\tau} t} + \varepsilon(t) \\
\end{eqnarray}

This decomposition transfers directly to the statistical model for measured signals $s_{j,t}$
\begin{equation}
s_{j,t} = \sum_{\ell \in \mathcal{K}_i} a_{\ell} \cdot e^{i 2\pi \frac{\ell}{\tau} t} + \varepsilon_t.
\end{equation}


\subsection{Estimating the spectral density}
Clustering the waves in the frequency domain also allows to use the well-developed theory of spectral densities of time series. For example, an for a white noise sequence each frequency is equally important ($\rightarrow$ uniform distribution); for the wave signal only very few frequencies are important. Furthermore, the important frequencies will be the low frequencies, not the high ones. This makes it easy to separate between signal and noise.

In practice the data of a wave form is a time series of length $T$, $(s_{i,1}, \ldots, s_{i,T})$; the Fourier coefficients at the Fourier frequencies $\omega_j = \frac{2 \pi j}{T}$ for $j = 0, \ldots, T-1$ are 
\begin{equation}
X_j = \sum_{n=0}^{T-1} S_i(n) e^{-\frac{2 \pi i}{T} j n} \quad \quad j = 0, \dots, T-1 
\end{equation}
The fast fourier transform (FFT) can achieve that computation in $\mathcal{T \log T}$ operations.


\begin{table}[!b]
\caption{\label{tab:notation} Notation used in this analysis.}
\begin{center} 
\begin{tabular}{ | l | l | l | }
 \hline 
$n_i$ & Neuron $i$ & $i = 1, \ldots, K$; $K$ unknown\\ 
$\mathcal{N}$ & collection of all neurons $\mathcal{N} = \lbrace n_1, \ldots, n_K \rbrace$ & \\
 \hline 
$S_i(t)$ & spike-signal from $n_i$ & $i=1,\ldots, K$, $t \in \R$ \\ 
$\mathcal{S}$ & collection of all spike-signal wave forms $\mathcal{S} =\lbrace S_1(t), \ldots, S_K(t) \rbrace$ & \\
\hline
$\boldsymbol{\alpha}^{(i)} = \lbrace \alpha_{\ell}^{(i)} \rbrace \in \C$ & Fourier coefficients of $S_i(t)$ & $\ell = 0, \pm 1,\pm2 , \ldots$ \\
$\mathcal{A}$ & collection of all sequences $\mathcal{A} =\lbrace \boldsymbol{\alpha}^{(1)}, \ldots, \boldsymbol{\alpha}^{(K)} \rbrace$ & \\
 \hline 
$s_{j,t}$ & $N > K$ measured signals & $j = 1, \ldots, N$, $t = 1,\ldots, T$ \\
$\mathbf{a}^{(j)} = \lbrace a_{\ell}^{(j)} \rbrace$ & Fourier coefficients of $s_{j,t}$ & $\ell = 0, 1, \ldots, T-1$ \\
 \hline 
 \end{tabular} 
 \end{center}
\end{table}


\begin{definition}[Discrete Fourier Transform]
For a sequence $(x_1, \ldots, x_T)$, define the discrete Fourier transform (DFT) as $(X(\omega_0), X(\omega_1), \ldots, X(\omega_{n-1}))$, where
\begin{equation}
X(\omega_k) = \frac{1}{\sqrt{T}} \sum_{t=1}^{T} x_t e^{-2 \pi i \omega_k t},
\end{equation}
and $\omega_k = \frac{k}{T}$ for $k=0, 1, \ldots, T-1$ are the Fourier frequencies.
\end{definition}

Since the Fourier basis $\lbrace e^{2 \pi i \omega_k t} \rbrace$ is an orthonomal sequence, the coordinates of $x_t$ in the Fourier basis are $X(\omega_k)$, i.e.\
\begin{equation}
x_t = \sum_{k=0}^{T-1} \innerprod{x_t, e_k} e_k = \sum_{k=0}^{T-1} X(\omega_k) e^{2 \pi i \omega_k t}.
\end{equation}



==> preamble.tex <==
\newcommand{\E}{\mathbb{E}}
\newcommand{\V}{\mathbb{V}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Prob}{\mathbb{P}}
\newcommand{\vnorm}[1]{\left|\left|#1\right|\right|}
\newcommand{\dx}[2]{\frac{\mathrm{d} #1}{\mathrm{d} #2}} 
\renewcommand\Re{\mathcal{R}}
\newcommand{\event}[1]{$\lbrace$ #1 $\rbrace$}


\newcommand{\SIM}[2]{\operatorname{sim}\left(#1 , #2 \right)} 
\newcommand{\DIST}[2]{\operatorname{dist}\left(#1 , #2 \right)} 
\newcommand{\logtwo}{\log_{2}}
\newcommand{\KL}[2]{\operatorname{KL}\left(#1 \mid \mid #2 \right)} 
\newcommand{\SymKLexp}[2]{\frac{\KL{p}{q} + \KL{q}{p}}{2}} 
\newcommand{\symKL}[2]{\operatorname{KL}_S\left(#1 \mid \mid #2 \right)} 
\newcommand{\expKL}[2]{\operatorname{KL}^{\gamma}\left(#1 \mid \mid #2 \right)} 
\newcommand{\innerprod}[1]{\langle #1 \rangle}

\usepackage{float}
\usepackage[authoryear,sort&compress,longnamesfirst]{natbib}
%\usepackage[left=2.2cm,top=2.2cm,right=2.2cm,bottom=2.2cm, includefoot]{geometry}
\usepackage[left=2cm,top=2cm,right=2cm,bottom=1.8cm, includefoot]{geometry}
%\usepackage[left=1cm,top=1cm,right=1cm,bottom=1cm, includefoot]{geometry}
\usepackage{amssymb, amsmath}
\usepackage{graphicx}
\usepackage{amsthm}
\usepackage{verbatim}
\usepackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
%\usepackage[nolists]{endfloat}
\usepackage{algorithm}
\usepackage[noend]{algorithmic}
\usepackage{tikz}
\usetikzlibrary{shapes,arrows}
\usepackage{fancyhdr}
\usepackage{url}
\usepackage{subfig}

\setlength{\marginparsep}{-0.5cm}
\setlength{\marginparwidth}{1.5 cm}
\newenvironment{edit}[2][Note]{\dag\marginpar{\tiny{\textbf{#1:} {#2}}}}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{acknowledgement}[theorem]{Acknowledgement}
\newtheorem{algorithmk}[theorem]{Algorithm}
\newtheorem{axiom}[theorem]{Axiom}
\newtheorem{case}[theorem]{Case}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{conclusion}[theorem]{Conclusion}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{criterion}[theorem]{Criterion}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{exercise}[theorem]{Exercise}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{solution}[theorem]{Solution}
\newtheorem{summary}[theorem]{Summary}



